Dynamical approach to chains of scatterers

Linear chains of quantum scatterers are studied in the process of lengthening, which is treated and analysed as a discrete dynamical system defined over the manifold of scattering matrices. Elementary properties of such dynamics relate the transport through the chain to the spectral properties of individual scatterers. For a single-scattering channel case some new light is shed on known transport properties of disordered and noisy chains, whereas translationally invariant case can be studied analytically in terms of a simple deterministic dynamical map. The many-channel case was studied numerically by examining the statistical properties of scatterers that correspond to a certain type of transport of the chain i.e. ballistic or (partially) localised.

==> Makefile <==
all: achain_doc.dvi

achain_doc.dvi: achain_doc.tex
	latex achain_doc
	latex achain_doc

achain_doc.ps: achain_doc.dvi
	dvips -Ppdf -G0 achain_doc

achain_doc.A4.ps: achain_doc.ps
	csh ~/scripts/psA4toA5 -duplex achain_doc.ps achain_doc.A4.ps
	
achain_doc.pdf: achain_doc.ps
	ps2pdf achain_doc.ps achain_doc.pdf

achain_doc.djvu: achain_doc.ps
	djvudigital achain_doc.ps

# my shortcuts

ps: achain_doc.ps

ps.A4: achain_doc.A4.ps

pdf: achain_doc.pdf

djvu: achain_doc.djvu

archive:
	tar -cvzf achain_doc.tar.gz  `bash search achain_doc.tex` \
	iopart*.cl* Makefile



